Planning in Markov Decision Processes with Gap-Dependent Sample Complexity

We propose MDP-GapE, a new trajectory-based Monte-Carlo Tree Search algorithm for planning in a Markov Decision Process in which transitions have a finite support. We prove an upper bound on the number of calls to the generative models needed for MDP-GapE to identify a near-optimal action with high probability. This problem-dependent sample complexity result is expressed in terms of the sub-optimality gaps of the state-action pairs that are visited during exploration. Our experiments reveal that MDP-GapE is also effective in practice, in contrast with other algorithms with sample complexity guarantees in the fixed-confidence setting, that are mostly theoretical.

==> main/sketchproof.tex <==
\subsection{Sketch of Proof for Theorem~\ref{thm:newthm}}

We present the proof of Theorem~\ref{thm:newthm}, with the proof of intermediate lemmas postponed to Appendix~\ref{app:FirstAnalysis}. We use the notation $\sigma_h=\sum_{i=0}^{h-1}\gamma^i$ to upper bound the discounted reward in $h$ steps.

Our proof relies on two important ingredients. The first is Lemma~\ref{lem:allinone}, which provides a relationship between the state-action gaps and the diameter of the confidence intervals on their value.
The statement in Lemma~\ref{lem:allinone} is a simple consequence of the optimistic selection rule for $h\geq 2$ and exploits some properties of UGapE for $h=1$.
% The first inequality in Lemma~\ref{lem:allinone} exploits the fact that for $h\geq 2$, the policy is optimistic, that is $U_h^t(s_h,\pi_h^{t+1}(s_h)) = \max_{a} U_h^t(s_h,a)$, while the second is a more sophisticated consequence of the fact that UGapE is used to select the first action.

\begin{lemma}\label{lem:allinone}
 If $\cE$ holds and $t < \tau_\delta$, for all  $h\in[H]$ and $s_h\in\cS_h(\pi^{t+1})$,
{\small\[\tilde{\Delta}_h(s_h,\pi_h^{t+1}(s_h)) \leq 2\left[U_h^t(s_h,\pi_h^{t+1}(s_h)) - L_h^t(s_h,\pi_h^{t+1}(s_h))\right].\]}
\end{lemma}
\noindent

The second ingredient is an inductive relationship which is crucial to upper bound the diameter $D_h^t(s_h,a_h) \eqdef U_h^t(s_h,a_h) - L_h^t(s_h,a_h)$ of the confidence intervals.
In the deterministic case, if we denote by $s_1,a_1,\dots,s_H,a_H$ the $(t+1)$-st trajectory, generated with the policy $\pi^{t+1}$, the following recursive relationship is a consequence of the optimistic selection starting at depth $2$:
{\small\begin{align}
D_h^t(s_h,a_h) &\leq \left(u_h^t(s_h,a_h)- \ell_h^t(s_h,a_h)\right) + \gamma D_{h+1}^t\left(s_{h+1}, a_{h+1}\right) \nonumber\\
& \leq \left[\sqrt{\frac{2\beta(n^t_h(s_h,a_h),\delta)}{n^t_h(s_h,a_h)}} \wedge 1 \right] + \gamma D_{h+1}^t(s_{h+1}, a_{h+1}),\label{eq:stepdeterministic}
\end{align}}
\hspace{-0.2cm} where the second inequality uses Pinskers's inequality (and uses the convention $1/0 = +\infty$). In the stochastic case, %the derivation are a bit more complicated and
the recursive bound %, stated in Lemma~\ref{lemma:difference},
involves a summation over possible next states.
\begin{lemma}\label{lemma:difference}
If $\cE$ holds, for all $h\in[H]$, $s_h\in\cS_h(\pi^{t+1})$ and $a_h$,
{\small \[D_h^t(s_h,a_h) \leq  \sigma_{H-h+1} \left[4 \sqrt{2}\sqrt{ \frac {\beta(n_h^t(s_h,a_h), \delta)} {n_h^t(s_h,a_h)} } \wedge 1\right]+ \gamma\sum_{s'} p_h(s'|s_h,a_h) D_{h+1}^t(s',\pi_{h+1}^{t+1}(s')).\]}
\end{lemma}

We now assume that the event $\cE$ holds and fix some $h \in [H]$ and some state-action pair $(s_h,a_h)$. For every $\ell \geq h$, we define $p^{\pi}_{h,\ell}(s,a | s_h,a_h)$ to be the probability that starting from $(s_h,a_h)$ in step $h$ and following $\pi$ thereafter, we end up in $(s,a)$ in step $\ell$. We use $p^{t}_{h,\ell}(s,a |s_h,a_h)$ as a shorthand for $p^{\pi^t}_{h,\ell}(s,a |s_h,a_h)$. This permits to define some notion of \emph{expected diameter in a future step} $\ell$ given that $(s_h,a_h)$ is visited at step $h$ under policy $\pi^{t+1}$. For every $(h,\ell) \in [H]^2$ such that $h\leq \ell$ we let
\[q^{t}_{h,\ell}(s_h,a_h) \eqdef \sum_{(s,a)} p^{t+1}_{h}(s_h,a_h)p^{t+1}_{h,\ell}\left(s,a | s_h,a_h\right) D^{t}_{\ell}(s,a).\]
On the one hand, $q^{t}_{h,h}(s_h,a_h) = p^{t+1}_{h}(s_h,a_h)D^{t}_{h}(s_h,a_h)$  and Lemma~\ref{lem:allinone} yields, for all $t<\tau$,
$q^{t}_{h,h}(s_h,a_h)\geq \tfrac{1}{2}p^{t+1}_{h}(s_h,a_h) \tilde\Delta_h(s_h,a_h)\;$.
On the other hand, using Lemma~\ref{lemma:difference}, one can prove that
{\small\[q^t_{h,h}(s_h,a_h) \leq \sum_{\ell = h}^{H} \gamma^{\ell - h}\sigma_{H-\ell+1}\sum_{(s,a)} p^{t+1}_{h}(s_h,a_h)p^{t+1}_{h,\ell}\left(s,a | s_h,a_h\right)\left[4 \sqrt{2}\sqrt{ \frac {\beta(n_{\ell}^t(s,a), \delta)} {n_{\ell}^t(s,a)} } \wedge 1\right]\;.\]}
Summing these inequalities for $t \in \{0,\tau-1\}$ permits to upper bound $\bar n_h^{\tau}(s_h,a_h) \tilde{\Delta}_h(s_h,a_h)$ by {\small
\begin{equation}2\sum_{\ell = h}^{H} \gamma^{\ell - h}\sigma_{H-\ell+1}\sum_{(s,a)}\sum_{t=0}^{\tau-1} p^{t+1}_{h}(s_h,a_h)p^{t+1}_{h,\ell}\left(s,a | s_h,a_h\right)\left[4 \sqrt{2}\sqrt{ \frac {\beta(n_{\ell}^t(s,a), \delta)} {n_{\ell}^t(s,a)} } \wedge 1\right]\label{ub:RHS}\,.\end{equation}}
\hspace{-0.2cm} Introducing the \emph{conditional pseudo-counts} $\bar n_{h,\ell}^{t}(s,a ; s_h,a_h)\eqdef\sum_{i=1}^{t}  p^{i}_{h}(s_h,a_h)p^{i}_{h,\ell}\left(s,a | s_h,a_h\right)$ and using that on the event $\cE^{\cnt} \supseteq \cE$ the counts are close to the pseudo-counts, one can prove:

\begin{lemma}\label{lemma:technicalCounts}
If the event $\cE^{\cnt}$ holds, $\left[\sqrt{ \tfrac {\beta(n_{\ell}^t(s,a), \delta)} {n_{\ell}^t(s,a)} } \wedge 1\right] \leq 2\sqrt{\tfrac{\beta(\overline{n}_{h,\ell}^t(s,a ; s_h,a_h), \delta)}{\overline{n}_{h,\ell}^t(s,a ; s_h,a_h) \vee 1}}$.
\end{lemma}

Note that the sum over $(s,a)$ in \eqref{ub:RHS} can be restricted to the set $\cS_{h,\ell}(s_h,a_h)$ of the $(BK)^{h - \ell}$ state-action pairs that can be reached from $(s_h,a_h)$ in step $\ell$. Using Lemma~\ref{lemma:technicalCounts} together with Lemma 19 in \cite{UCRL10} and the fact that $n_h^{\tau}(s_h,a_h) = \sum_{(s,a) \in \cS_{h,\ell}(s_h,a_h)} n_{n,\ell}^{\tau}(s,a ; s_h,a_h)$, we get
{\small
\begin{eqnarray*}
\eqref{ub:RHS} &\leq& 16\sqrt{2}\sqrt{\beta(\bar n_h^{\tau}(s_h,a_h),\delta)}\sum_{\ell = h}^{H} \gamma^{\ell - h}\sigma_{H-\ell+1}\sum_{(s,a)\in\cS_{h,\ell}(s_h,a_h)}\sum_{t=0}^{T} \frac{\bar n_{h,\ell}^{t+1}(s,a ; s_h,a_h) - \bar n_{h,\ell}^{t+1}(s,a ; s_h,a_h) }{\bar n_{h,\ell}^{t}(s,a ; s_h,a_h) \vee 1} \\
& \leq & 16\sqrt{2}(1+\sqrt{2})\sqrt{\beta(\bar n_h^{\tau}(s_h,a_h),\delta)}\sum_{\ell = h}^{H} \gamma^{\ell - h}\sigma_{H-\ell+1}\sum_{(s,a)\in\cS_{h,\ell}(s_h,a_h)}\sqrt{\bar n_{h,k}^{\tau}(s,a ; s_h,a_h)} \\
& \leq & 16\sqrt{2}(1+\sqrt{2})\sqrt{\beta(\bar n_{h}^{\tau}(s_h,a_h),\delta)}\sum_{\ell = h}^{H} \gamma^{\ell - h}\sigma_{H-\ell+1}\sqrt{(BK)^{\ell - h}}\sqrt{\bar n_h^{\tau}(s_h,a_h)}\;.
\end{eqnarray*}}
\hspace{-0.2cm} The conclusion follows as the sum over $h$ can be upper bounded by Lemma~\ref{lemma:constants} in Appendix~\ref{subsec:detail}.

